Abstract Scene Graphs: Formalizing and Monitoring Spatial Properties of Automated Driving Functions

Automated Driving Functions (ADFs) need to comply with spatial properties of varied complexity while driving on public roads. Since such situations are safety-critical in nature, it is necessary to continuously check ADFs for compliance with their spatial properties. Due to their complexity, such spatial properties need to be formalized to enable their automated checking. Scene Graphs (SGs) allow for an explicit structured representation of objects present in a traffic scene and their spatial relationships to each other. In this paper, we build upon the SG construct and propose the Abstract Scene Graph (ASG) formalism to formalize spatial properties of ADFs. We show using real-world examples how spatial properties can be formalized using ASGs. Finally, we present a framework that uses ASGs to perform Runtime Monitoring of ADFs. To this end, we also show algorithmically how a spatial property formalized as an ASG can be satisfied by ADF system behaviour.

==> eptcsdata.tex <==
\providecommand{\firstpage}{3}
\providecommand{\publicationstatus}{Matt Luckcuck, Maike Schwammberger \& Mengwei Xu (Eds.):\\
Seventh International Workshop on Formal Methods\\
for Autonomous Systems (FMAS 2025)\\
EPTCS 436, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.436.3}{10.4204/EPTCS.436.3}}
\pdfoutput=1

